Evolution of Directed Triangle Motifs in the Google+ OSN

Motifs are a fundamental building block and distinguishing feature of networks. While characteristic motif distribution have been found in many networks, very little is known today about the evolution of network motifs. This paper studies the most important motifs in social networks, triangles, and how directed triangle motifs change over time. Our chosen subject is one of the largest Online Social Networks, Google+. Google+ has two distinguishing features that make it particularly interesting: (1) it is a directed network, which yields a rich set of triangle motifs, and (2) it is a young and fast evolving network, whose role in the OSN space is still not fully understood. For the purpose of this study, we crawled the network over a time period of six weeks, collecting several snapshots. We find that some triangle types display significant dynamics, e.g., for some specific initial types, up to 20% of the instances evolve to other types. Due to the fast growth of the OSN in the observed time period, many new triangles emerge. We also observe that many triangles evolve into less-connected motifs (with less edges), suggesting that growth also comes with pruning. We complement the topological study by also considering publicly available user profile data (mostly geographic locations). The corresponding results shed some light on the semantics of the triangle motifs. Indeed, we find that users in more symmetric triangle motifs live closer together, indicating more personal relationships. In contrast, asymmetric links in motifs often point to faraway users with a high in-degree (celebrities).

==> bigtable.tex <==
\begin{table}[h!]
  \centering
  \begin{tabular}{| c | c | c | c | c | c | c | c | c | c | c | c | c | c |}
    \hline
     &
   \begin{minipage}{.03\textwidth}
      \includegraphics[height=4mm]{tri-1}
    \end{minipage}
    &
   \begin{minipage}{.03\textwidth}
      \includegraphics[height=4mm]{tri-2}
    \end{minipage}
&
   \begin{minipage}{.03\textwidth}
      \includegraphics[height=4mm]{tri-3}
    \end{minipage}
    &
   \begin{minipage}{.03\textwidth}
      \includegraphics[height=4mm]{tri-4}
    \end{minipage}
    &
   \begin{minipage}{.03\textwidth}
      \includegraphics[height=4mm]{tri-5}
    \end{minipage}
&
   \begin{minipage}{.03\textwidth}
      \includegraphics[height=4mm]{tri-6}
    \end{minipage}
&
    \begin{minipage}{.03\textwidth}
      \includegraphics[height=4mm]{tri-7}
    \end{minipage}
&
    \begin{minipage}{.03\textwidth}
      \includegraphics[height=4mm]{tri-8}
    \end{minipage}
&
    \begin{minipage}{.03\textwidth}
      \includegraphics[height=4mm]{tri-9}
    \end{minipage}
&
    \begin{minipage}{.03\textwidth}
      \includegraphics[height=4mm]{tri-10}
    \end{minipage}
&
    \begin{minipage}{.03\textwidth}
      \includegraphics[height=4mm]{tri-11}
    \end{minipage}
&
    \begin{minipage}{.03\textwidth}
      \includegraphics[height=4mm]{tri-12}
    \end{minipage}
&
    \begin{minipage}{.03\textwidth}
      \includegraphics[height=4mm]{tri-13}
    \end{minipage}
        \\ \hline
    \begin{minipage}{.03\textwidth}
      \includegraphics[height=4mm]{tri-1}
    \end{minipage} & nix & nix & nix & nix & nix & nix & nix & nix & nix & nix & nix & nix & nix
        \\ \hline
            \begin{minipage}{.03\textwidth}
      \includegraphics[height=4mm]{tri-2}
    \end{minipage} & nix & nix & nix & nix & nix & nix & nix & nix & nix & nix & nix & nix & nix
        \\ \hline
            \begin{minipage}{.03\textwidth}
      \includegraphics[height=4mm]{tri-3}
    \end{minipage} & nix & nix & nix & nix & nix & nix & nix & nix & nix & nix & nix & nix & nix
        \\ \hline
            \begin{minipage}{.03\textwidth}
      \includegraphics[height=4mm]{tri-4}
    \end{minipage} & nix & nix & nix & nix & nix & nix & nix & nix & nix & nix & nix & nix & nix
        \\ \hline
            \begin{minipage}{.03\textwidth}
      \includegraphics[height=4mm]{tri-5}
    \end{minipage} & nix & nix & nix & nix & nix & nix & nix & nix & nix & nix & nix & nix & nix
        \\ \hline
            \begin{minipage}{.03\textwidth}
      \includegraphics[height=4mm]{tri-6}
    \end{minipage} & nix & nix & nix & nix & nix & nix & nix & nix & nix & nix & nix & nix & nix
        \\ \hline
            \begin{minipage}{.03\textwidth}
      \includegraphics[height=4mm]{tri-7}
    \end{minipage} & nix & nix & nix & nix & nix & nix & nix & nix & nix & nix & nix & nix & nix
        \\ \hline
            \begin{minipage}{.03\textwidth}
      \includegraphics[height=4mm]{tri-8}
    \end{minipage} & nix & nix & nix & nix & nix & nix & nix & nix & nix & nix & nix & nix & nix
        \\ \hline
            \begin{minipage}{.03\textwidth}
      \includegraphics[height=4mm]{tri-9}
    \end{minipage} & nix & nix & nix & nix & nix & nix & nix & nix & nix & nix & nix & nix & nix
        \\ \hline
            \begin{minipage}{.03\textwidth}
      \includegraphics[height=4mm]{tri-10}
    \end{minipage} & nix & nix & nix & nix & nix & nix & nix & nix & nix & nix & nix & nix & nix
        \\ \hline
            \begin{minipage}{.03\textwidth}
      \includegraphics[height=4mm]{tri-11}
    \end{minipage} & nix & nix & nix & nix & nix & nix & nix & nix & nix & nix & nix & nix & nix
        \\ \hline
            \begin{minipage}{.03\textwidth}
      \includegraphics[height=4mm]{tri-12}
    \end{minipage} & nix & nix & nix & nix & nix & nix & nix & nix & nix & nix & nix & nix & nix
        \\ \hline
            \begin{minipage}{.03\textwidth}
      \includegraphics[height=4mm]{tri-13}
    \end{minipage} & nix & nix & nix & nix & nix & nix & nix & nix & nix & nix & nix & nix & nix
        \\ \hline
%    &
%    nix
%    &
%    nix
%    &
%    nix \\
%    \hline
  \end{tabular}
  \caption{Triangle Transitions}\label{tbl:tritra}
\end{table}


